Desiree - a Refinement Calculus for Requirements Engineering

The requirements elicited from stakeholders suffer from various afflictions, including informality, incompleteness, ambiguity, vagueness, inconsistencies, and more. It is the task of requirements engineering (RE) processes to derive from these an eligible (formal, complete enough, unambiguous, consistent, measurable, satisfiable, modifiable and traceable) requirements specification that truly captures stakeholder needs. We propose Desiree, a refinement calculus for systematically transforming stakeholder require-ments into an eligible specification. The core of the calculus is a rich set of requirements operators that iteratively transform stakeholder requirements by strengthening or weakening them, thereby reducing incompleteness, removing ambiguities and vagueness, eliminating unattainability and conflicts, turning them into an eligible specification. The framework also includes an ontology for modeling and classifying requirements, a description-based language for representing requirements, as well as a systematic method for applying the concepts and operators. In addition, we define the semantics of the requirements concepts and operators, and develop a graphical modeling tool in support of the entire framework. To evaluate our proposal, we have conducted a series of empirical evaluations, including an ontology evaluation by classifying a large public requirements set, a language evaluation by rewriting the large set of requirements using our description-based syntax, a method evaluation through a realistic case study, and an evaluation of the entire framework through three controlled experiments. The results of our evaluations show that our ontology, language, and method are adequate in capturing requirements in practice, and offer strong evidence that with sufficient training, our framework indeed helps people conduct more effective requirements engineering.

==> temp.tex <==
\section{Semantics of \emph{Desiree}}
\label{sec:desiree_temp}
\vspace{12pt}
\noindent \emph{\textbf{Translation of requirements concepts.}} In general, every requirement (FG, CTG, QG, F, FC, QC, SC, and DA) are initially stated using natural language (NL). These early requirements are refined into elements with a corresponding structured syntax in our \emph{Desiree} framework (we call them ``early requirements'' or ``stakeholder requirements''  because they are what we start with).

In \emph{Desiree}, early requirements are mere atomic propositions; and the instances of an early requirement are all the corresponding problem situations (i.e., all the cases when the specific intention is instantiated). For example, for the propositional requirement ``schedule a meeting'', the instances are all the specific requests for a meeting. Further, such requirements can be organized into a subsumption hierarchy by using ``$E_1 :< E_2$'' statements. For example, given $F_1$ ``download contact information for clients'' and $F_2$ ``download clients' contact information'', we can organize them by simply denoting ``$F_2 :< F_1$'' (here $F_1$ is ambiguous since it has another interpretation ``download contact information in the sake of clients'', hence we have only ``$F_2 :< F_1$'' but not the reverse).
%while later ones, derived through refinements, are structured ones having a more elaborate subsumption relation.
%for the two NL functions

%Two subclasses of G, namely FG and CTG, are formulae of the form as $Desc$ in Eq.~\ref{eq:eq_semantics_subsumption}, where \emph{C} and \emph{D} are concepts defined using our language. The same kinds of formulae are used to express FCs, SCs, and DAs. The semantics of such formulae are closed formulae as $AX_{Desc}$ in Eq.~\ref{eq:eq_semantics_subsumption}, and the translation of such formulae to DL axioms can be done according to $DLAxiom_{Desc}$ in Eq.~\ref{eq:eq_semantics_subsumption}.
%The same kinds of formulae are used to express FCs, SCs, and DAs.
\emph{Desiree} elements, derived through refinements, are structurally specified. Especially, FGs, CTGs, FCs, SCs, and DAs are formulae of the form as $Desc$ in Eq.~\ref{eq:eq_semantics_subsumption}, where \emph{C} and \emph{D} are concepts defined using our language. The semantics of such formulae are closed formulae as $AX_{Desc}$ in Eq.~\ref{eq:eq_semantics_subsumption}, and the translation of such formulae to DL axioms can be done according to $DLAxiom_{Desc}$ in Eq.~\ref{eq:eq_semantics_subsumption}. For example, the semantics of the FC ``$FC_1$ := Data\_table $:<$ $<$accessed\_by: ONLY Manager$>$'' will then emerge as ``$\forall$\emph{x}/Data\_table $\forall$\emph{y} accessed\_by (\emph{x}, \emph{y}) $\rightarrow$ \emph{y} $\in$ Manager'', where ``$\forall x/C$'' is a shorthand for ``$\forall x.x \in C$''. Further, this FC will be translated to the DL axiom ``Data\_table $\sqsubseteq$ $\forall$ accessed\_by.Manager''.\\
\begin{equation}\label{eq:eq_semantics_subsumption}
    \begin{aligned}
        Desc := \; & C :< D \\
        AX_{Desc} \equiv \; & \forall x.  x \in  \bm{T}(C) \rightarrow  x \in  \bm{T}(D) \\
        DLAxiom_{Desc} \equiv \; & \bm{L} (C) \sqsubseteq \bm{L} (D) \\
    \end{aligned}
\end{equation}
%DLConcept_{Desc} \equiv \; & \exists subsumee.\bm{L} (C) \sqcap \exists subsumer.\bm{L} (D)

In addition, we translate formulae of the syntactic form ``C $:<$ D'' in to DL concepts as $DLConcept_{Desc}$ in Eq.~\ref{eq:eq_subsumption_concept}, where ``subsumee'' and ``subsumer'' are reserved object properties that have ``$\bm{L} (C)$'' and ``$\bm{L} (D)$'' as ranges (fillers), respectively. For example, we translate the above $FC_1$ into a DL concept ``$\exists$ subsumee.Data\_table $\sqcap$ subsumer.($\forall$ accessed\_by.Manager)''.
\begin{equation}\label{eq:eq_subsumption_concept}
    \begin{aligned}
        DLConcept_{Desc} \equiv \; & \exists subsumee.\bm{L} (C) \sqcap \exists subsumer.\bm{L} (D)
    \end{aligned}
\end{equation}

%At the same time, we associate with this subsumption axiom a DL concept ``$\exists$ subsumee.Data\_table $\sqcap$ subsumer.($\forall$ accessed\_by.Manager)''. In the rest of this section,  we focus on the semantics of the other three kinds of requirement concepts, namely Functions, QGs and QCs.
This is mainly for representing the subsumption between input and output elements of requirements operators (to be discussed later in Section~\ref{sec:semantics_operator}). For example, if an FC in the form ``$FC_1 := A :< B$'' is reduced to another ``$FC_2 := C :< D$'', we can organize $FC_1$ and $FC_2$ in a subsumption hierarchy if they can be translated into DL concepts as in Eq.~\ref{eq:eq_subsumption_concept} (e.g., $FC_2 :< FC_1$), and can not do so if $F_1$ and $F_2$ are in their original forms, which represent assertions.

In the rest of this section,  we focus on the semantics of the other three kinds of requirement concepts, namely Functions, QGs and QCs. 

==> translateF.tex <==
\vspace{6pt}
\noindent \emph{\textbf{Translation of Functions.}} In \emph{Desiree}, a function description consists of a function name and a list of optional slot-description pairs (\emph{SlotDs}). Ontologically, it represents a set of manifestations (i.e., runs) of a capability. For example, the expression ``$F_1$ := Activate $<$actor: Manager$>$$<$object: Debit\_card$>$'' says that each run of $F_1$ is an activation with a manager as its actor and a debit card as its object. Our description translation gives the semantics of $F_1$ as $AX_{F_1}$ in Eq. \ref{eq:eq_semantics_f_example}. Note that ``actor'' and ``object'' are functional slots, and are translated into functional object properties in DL.
%, where ``$|M|$'' denotes the cardinality of a set ``$M$'', and ``$s(x, M)$'' represents a set ``$\{y | (x, y) \in s \land y \in M\}$''.
%Note that $F_1$ can only have managers as its actor; that is, if not explicitly specified, other user roles are not allowed to activate debit cards. The same interpretation applies to its object (and other slots, if exist).
\begin{equation}\label{eq:eq_semantics_f_example}
    %\small
    \begin{aligned}
    AX_{F_1} \equiv \:  & \forall x.F_1 (x) \rightarrow Activate (x)   \\
                    & \land (\forall y. actor (x, y) \rightarrow y \in Manager) \land \exists y.actor(x,y) \\
                    & \land (\forall y . object (x, y) \rightarrow y \in Debit\_card) \land \exists y.object(x,y)\\
    \end{aligned}
\end{equation}
%|actor(x, Manager)| = 1
%|object(x, Debit\_card)|=1
\begin{comment}
\begin{equation}\label{eq:eq_semantics_f_example}
    %\small
    \begin{aligned}
    AX_{F_1} \equiv \; &\forall x.F_1(x)\rightarrow Activate (x) \land \forall y. actor(x, y) \rightarrow y \in Manager  \\
                    & \land \forall y . object (x, y) \rightarrow y \in Debit\_card \\
    \end{aligned}
\end{equation}
\end{comment}

%(``$s$'' is a functional slot)
In general, the semantics of a function specified as ``$F_e$ := \emph{FName} $<s: D>$'' (``$s$'' is a functional slot) can be generalized as in Eq. \ref{eq:eq_semantics_f_general}.
\begin{equation}\label{eq:eq_semantics_f_general}
    %\small
    \begin{aligned}
    AX_{F_e} \equiv \;  & \forall x/F_e \rightarrow FName(x)\\
                        & \land (\forall y.s(x,y) \rightarrow y \in \bm{T}(D)) \land \exists y.s(x,y)
    \end{aligned}
\end{equation}
%\land |s(x,\bm{T}(D))|=1
\begin{comment}
\begin{equation}\label{eq:eq_semantics_f_general}
    %\small
    \begin{aligned}
    AX_{F_e} \equiv \;  & \forall x/F_e \rightarrow FName(x) \land \forall y.s(x,y) \rightarrow y \in \bm{T}(D)
    \end{aligned}
\end{equation}
\end{comment}

%which has a necessary condition ``$\forall$ actor.Thing $\sqcap$ $\forall$ object.Thing'' (i.e., ``Function $\sqsubseteq$ $\forall$ actor.Thing $\sqcap$ $\forall$ object.Thing'') that constrains the basic slots (``actor'' and ``object''),
% which has a necessary condition ``$\forall$ inheres\_in.SubjT $\sqcap$ $\exists$ inheres\_in.SubjT'' (i.e., ``Function $\sqsubseteq$ $\forall$ inheres\_in.SubjT $\sqcap$ $\exists$ inheres\_in.SubjT''),
When translating a function description to DL, the function name will be a sub-class of ``{\textbf{Function}}'', and the slot-description pairs will be translated according to rule $1 \sim 9$ in Table \ref{tab:semantics_descriptions}. For example, the function description $F_1$ above will result in the declaration of concept $F_1$ as shown in Eq. \ref{eq:eq_translation_f_example}.
%$DL_{F_1}$
\begin{equation}\label{eq:eq_translation_f_example}
    \begin{aligned}
        F_1 \; \equiv \;& \textbf{Function} \sqcap Activate \\
                        &\sqcap \forall actor.Manager \sqcap \exists actor.Manager \\
                        &\sqcap \forall object.Debit\_card \sqcap \exists object.Debit\_card \\
    \end{aligned}
\end{equation}
\begin{comment}
\begin{equation}\label{eq:eq_translation_f_example}
    \begin{aligned}
        F_1 \; \equiv \;& \textbf{Function} \sqcap Activate \sqcap \forall actor.Manager \sqcap \forall object.Debit\_card \\
    \end{aligned}
\end{equation}
\end{comment}

Generally, a function description $F_e$ as above will be translated into a DL concept $F_e$ as in Eq. \ref{eq:eq_translation_f_general}. %(``$s$'' is a functional property).
\begin{equation}\label{eq:eq_translation_f_general}
    \begin{aligned}
       {F_e} \; \equiv \;& \textbf{Function} \sqcap FName \sqcap \forall s.\bm{T}(D) \sqcap \exists s.\bm{T}(D)
    \end{aligned}
\end{equation}

%and hence does not have a truth value.
%we can simply replace ``SubjT'' with ``\{the\_system\}'', obtaining the following assertion: ``\{F\} $:<$
A function expression is a description, not an assertion. To assert whether a function has been implemented or not, we add an assertion $Assert\_F$ for each function description $F$ as in Eq. \ref{eq:eq_assert_funtion_inheresubj}, where ``inheres\_in'' is a functional slot. We say that a function has been implemented if there is such a function individual $\{F\}$ that inheres in the subject of concern, often the system to be designed, but can also be other agents in the software ecosystem, e.g., developers, testers and maintainers. For example, to assert the ``activate debit\_card'' function $F_1$, the subject of which is the system-to-be, we use the following assertion: ``\{$F_1$\} $:<$ $<$inheres\_in: \{the\_system\}$>$''. The semantics and the corresponding DL translation of such assertions are generalized in Eq. \ref{eq:eq_assert_funtion_inheresubj}. \\
\begin{equation}\label{eq:eq_assert_funtion_inheresubj}
    \begin{aligned}
       Assert\_F := \; & \{F\} :< \; <inheres\_in: SubjT> \\
       AX_{Assert\_F} := \; & \forall x/\{F\} \; (\forall y.inheres\_in (x, y) \rightarrow y \in SubjT) \\
                            & \land \exists y. inheres\_in(x, y)\\
                           %& \land |inheres\_in(x, \{the\_system\})| = 1\\
       DL_{Assert\_F} := \; & \{F\} \sqsubseteq \forall \;inheres\_in.SubjT \sqcap \exists \;inheres\_in.SubjT
                            %1 \; inheres\_in.\{the\_system\}
    \end{aligned}
\end{equation}
%Assert\_F := \; & SubjT :< <has\_function: \{F\}>
\begin{comment}
\begin{equation}\label{eq:eq_assert_funtion}
    \begin{aligned}
       Assert\_F := \; & \{F\} :< <inheres\_in: \{the\_system\}> \\
       AX_{Assert\_F} := \; & \forall x/\{F\} \; (\forall y \; inheres\_in (x, y) \rightarrow y \in \{the\_system\}) \\
                            & \land \exists y. inheres\_in(x, y)\\
                           %& \land |inheres\_in(x, \{the\_system\})| = 1\\
       DL_{Assert\_F} := \; & \{F\} \sqsubseteq \forall \;inheres\_in.\{the\_system\} \sqcap \exists \;inheres\_in.\{the\_system\}
                            %1 \; inheres\_in.\{the\_system\}
    \end{aligned}
\end{equation}
\begin{equation}\label{eq:eq_assert_funtion}
    \begin{aligned}
       Assert\_F := \; & \{F\} :< <inheres\_in: \{the\_system\}> \\
       AX_{Assert\_F} := \; & \forall x/\{F\} \; (\forall y \; inheres\_in (x, y) \rightarrow y \in \{the\_system\}) \\
                            & \land |inheres\_in(x, \{the\_system\})| = 1\\
       DL_{Assert\_F} := \; & \{F\} \sqsubseteq \forall \; inheres\_in.\{the\_system\} \sqcap 1 \; inheres\_in.\{the\_system\}
    \end{aligned}
\end{equation}
\end{comment}

Alternative, we can assert that a subject of concern shall have a desired function (capability), as shown in Eq. \ref{eq:eq_assert_funtion_hasf}, where ``has\_function'' is the inverse property of ``inheres\_in''. For example, ``\{the\_system\} $:<$ $<$has\_function: EXIST \{$F_1$\}$>$''.
\begin{equation}\label{eq:eq_assert_funtion_hasf}
    \begin{aligned}
       Assert\_F := \; & SubjT :< \; <has\_function: EXIST \; \{F\}>  \\
       AX_{Assert\_F} := \; & \forall s/SubjT \; \exists y.has\_function(s, y) \land y \in \{F\} \\
       DL_{Assert\_F} := \; & SubjT \sqsubseteq \exists \;has\_function.\{F\}
    \end{aligned}
\end{equation}

Note that a function individual can only inheres in one particular subject, while a subject could possess many function individuals. Therefore, we use ``SubjT $:<$ $<$has\_function: EXIST \{F\} $>$'' instead of ``SubjT $:<$ $<$has\_function: \{F\}$>$'': we can not constrain all the function individuals possessed by a subject to be of the same type; i.e., we can not have ``$\forall$ s/SubjT ($\forall$ y.has\_function(s, y) $\rightarrow$ y $\in$ \{F\})'', which is part of the semantics of ``SubjT $:<$ $<$has\_function: \{F\}$>$''.

%In addition, the distinction between a function individual $\{F\}$ and a set of its executions $F$ allows us to specifying requirement on the function (capability) itself besides its executions. For instance, we can require the ``schedule meetings'' function of a meeting scheduler to be easy to learn (e.g., $QG_{si}$ in Eq. \ref{eq:eq_findividual_fruns}), and also require its executions to be fast (e.g., $QG_{se}$ in Eq. \ref{eq:eq_findividual_fruns}).
%on not only its manifestations (executions), but also the function (capability) itself
In addition, the distinction between a function individual $\{F\}$ and its manifestations $F$ allows us to specify requirements on the function (capability) itself. For example, on one hand, we can require the ``schedule meeting'' function of a meeting scheduler (its manifestations, i.e., executions) to be fast; on the other hand, we can also require the function (capability) itself to be easy to learn. These two requirements can be captured as $QG_{se}$ and $QG_{si}$ in Eq. \ref{eq:eq_findividual_fruns}, respectively. Their semantics will be discussed later.
%For instance, ``the schedule meeting function of the meeting scheduler shall be easy to learn''. This example can be captured as $QG_{si}$ in Eq. \ref{eq:eq_findividual_fruns}, the semantics of which will be discussed in the sequel.
%Here, we are interested in the functionality itself, not its executions.
%and also require its executions to be fast (e.g., $QG_{se}$ in Eq. \ref{eq:eq_findividual_fruns}).
\begin{equation}\label{eq:eq_findividual_fruns}
    \begin{aligned}
    F_s := & \; Schedule <actor: Organizer><object: Meeting>\\
    QG_{se} := & \; Processing\_time (F_s) :: Fast \\
    QG_{si} := & \; Learnability (\{F_s\}) :: Good
    \end{aligned}
\end{equation}
%``the scheduling function should be easy to use''. This example will be captured as a QG ``Operability (\{Scheduling\}) :: Easy'', the translation of which will be discussed in the sequel.

%``$\forall$\emph{s}/File\_search, $\forall$\emph{q}/Processing\_time, inheres\_in(\emph{q}, \emph{s}) $\rightarrow$ has\_value\_in(\emph{q}, time\_region (\emph{x}, 0, 30, \emph{sec.}))'' 
